Node Connectivity Augmentation of Highly Connected Graphs

Node-connectivity augmentation is a fundamental network design problem. We are given a $k$-node connected graph $G$ together with an additional set of links, and the goal is to add a cheap subset of links to $G$ to make it $(k+1)$-node connected. In this work, we characterize completely the computational complexity status of the problem, by showing hardness for all values of $k$ which were not addressed previously in the literature. We then focus on $k$-node connectivity augmentation for $k=n-4$, which corresponds to the highest value of $k$ for which the problem is NP-hard. We improve over the previously best known approximation bounds for this problem, by developing a $\frac{3}{2}$-approximation algorithm for the weighted setting, and a $\frac{4}{3}$-approximation algorithm for the unweighted setting.

==> 3.weighted_Hardness.tex <==
\section{ Hardness for weighted case}

Based on \cite{BERCZI2012565}. 

Can view the problem as a maximization problem. For \(n-3\)-connectivity, the problem is equivalent to finding a maximum weight square free \(2\)-matching in the complement graph, where we interpret edges that are not links as having "very large" cost, and all others that correspond to links as having cost equal to the link. 

\begin{lemma}
    The weighted square-free 2-matching problem is NP-hard even if the given graph is cubic, bipartite, and planar
\end{lemma}
This is proven by first proving the following lemma for \(2\)-factors.

\begin{lemma}
    The weighted square-free 2-factor problem is NP-hard even if the given graph is cubic, bipartite, and planar
\end{lemma}

They prove this result by a reduction from and instance of independent set problem in cubic, bipartite, planar graphs \(G(V,E)\) to the weighted square-free 2-factor problem. 

We get a weighted square-free 2-factor problem instance \(G'(V',E')\) as follows. 

For every edge \(e=uv\in E\), we get vertices 
\begin{align*}
    V^e \coloneqq \{&u^e_1, u^e_2, u^e_3, u^e_4, v^e_1, v^e_2, v^e_3, v^e_4\}\\
    E^e \coloneqq \{&u^e_1u^e_2, u^e_2u^e_3, u^e_3u^e_4, u^e_4u^e_1, v^e_1v^e_2,\\& v^e_2v^e_3, v^e_3v^e_4, v^e_4v^e_1, v^e_3u^e_4, v^e_4u^e_3\}
\end{align*}

For every vertex \(v\) adjacent to edges \(e_1,e_2,e_3\), we get the following edges
\begin{align*}
    E^v \coloneqq \{ v_1^{e_1}v_2^{e_1}, v_2^{e_1}v_1^{e_2}, v_1^{e_2}v_2^{e_2}, v_2^{e_2}v_1^{e_3}, v_2^{e_3}v_1^{e_1}\}
\end{align*}

Then \(V' = \bigcup V^v\) and \(E' = \bigcup E^e \bigcup E^v\). 

We assign costs as follows  for \(e'\in E'\)
\[
    w(e') = \left \{\begin{array}{@{}ll@{}}
        L & \text{if } e'= u_1^e u_2^e, v_1^ev_2^e, u_3^ev_4^e, v_3^eu_4^e, \text{for some } e=uv\in E\\
        1, & \text{if } e'\in E^v \text{ for some }  v\in V\\
        0, & \text{else}
        \end{array}\right\}
\]
Where \(L\geq 3n +1 \).

They then prove the following 
\begin{claim}
    The original graph \(G = (V, E)\) has an independent set of size \(k\) if and only if \(G' = (V', E')\) contains a square-free 2-factor whose total weight is \(4|E|L + 3k\)
\end{claim}
Key to the proof of this claim is the observation that any optimal 2-factor \(M\) must contain every edge of weight \(L\), and this restricts the edges of \(E^e\) that can be in the factor. In particular, there are three forms 

\begin{equation*}
    M\cup E^e = \left \{\begin{array}{@{}ll@{}}
        E^e \backslash \{ u_3^eu_4^e, v_3^ev_4^e\}\\
        E^e \backslash \{u^e_1u^e_4, u^e_2u^e_3, v^e_3v^e_4\}\\
        E^e \backslash \{v^e_1v^e_4, v^e_2v^e_3, u^e_3u^e_4 \}
        \end{array}\right\}
\end{equation*}


\subsection{ Extending to n-o(n)}
We will show that the weighed \(n-d\)-augmentation problem is as hard as the independent set problem. This will be done in a similar way to the case when \(d=4\). We will show this by showing a that a different problem is as hard as the independent set and then show that the hardness can be derived from that. 

Given a \(n-d\)-augmentation problem instance \(G'=(V,E)\), we consider the complement of $G'$, which we denote by $G$. The problem of augmenting $G'$ to be $n-d+1$-connected is equivalent to finding a $d-2$-matching of $G$ that is $K_{i,d-i}$ free for $i=1,\dots, d/2$.

% We call these $K_{i,d-i}$ subgraphs \emph{obstructions}.

Given an independent set problem instance \(G= (V, E)\) in a cubic graph, we construct a graph $\bar G$ that will be an instance of the weighted, obstruction free, $d-2$-factor problem. 

For every $e=uv \in E$, we will define a set of vertices, $V^e$, and edges $E^e$. First we have vertices $\{u^e_1, u^e_2, u^e_3, u^e_4, v^e_1, v^e_2, v^e_3, v^e_4\} \subseteq V^e$, and $\{ v_1^{e_1}v_2^{e_2}, v_1^{e_2}v_2^{e_3}, v_1^{e_3}v_2^{e_1}\} \subseteq E^e$. We also define complete graphs on vertices $A^e= \{a_1^e, \dots, a_{d-4}^e\}$ and $B^e = \{b_1^e, \dots, b_{d-4}^e\}$. Then $A^e\cup B^e \subseteq V$, and $E^e$ contains the edges of the complete graph on $A^e$ and $B^e$.

Consider $v\in V$, since $G$ is cubic, $v$ is incident to edges $e_1, e_2, e_3$. Then \(\{ v_1^{e_1},v_2^{e_1}, v_1^{e_2},v_2^{e_2}, v_1^{e_3}v_2^{e_3}\} \subseteq V^v\) and \(\{ v_1^{e_1}v_2^{e_1}, v_2^{e_1}v_1^{e_2}, v_1^{e_2}v_2^{e_2}, v_2^{e_2}v_1^{e_3}, v_2^{e_3}v_1^{e_1}\} \subseteq E^v\). We also define complete graphs on vertices $C^v = \{c_1^v, \dots, c_{d-4}^v\} \subseteq V^v$ and $D^v = \{d_1^v,\dots d_{d-4}^v\}\subseteq V^v$. 

We define $G' = (\cup_{v\in V} V^v \cup_{e\in E} V^e, \cup_{v\in V}E^v \cup_{e\in E} E^e)$.


We assign edge weights as follows for $e' \in E'$
\begin{equation}
    w(e') =
        \begin{cases}
            L & \text{if } e' \text{ incident to a node in } A^e, B^e, C^e, D^e\\
            L & \text{if } e'= u_1^e u_2^e, v_1^ev_2^e, u_3^ev_4^e, v_3^eu_4^e, \text{for some } e=uv\in E\\
            1 & \text{if } e'\in E^v \text{ for some } v\in V\\
            0 & \text{else}
        \end{cases}
\end{equation}




% For every $e=uv \in E$, we will add $A^u = K_{k-3}$, with vertices $\{a_1, \dots, a_{k-3}\}$ and $B^u = K_{k-3}$, with vertices $\{b_1, \dots, b_{k-3}\}$. We will also add edges $u_3^ea_i$ and $v_4^ea_i$ for $i=1,\dots,k-3$, and edges $v_3^eb_i$ and $u_4^eb_i$ for $i=1, \dots, k-3$. We also add edges $a_ib_i$ for $i=1,\dots, k-3$. Each of these edges will have cost $L$. 

% For each $v\in V$ that is incident to edges $e_1, e_2,e_3\in E$, we also add $C^v= K_{k-3}$ and $D^v = K_{k-3}$. Three vertices of the cycle are adjacent to every node of $C^v$ and the other three are adjacent to all of $D^v$. All of these edges are cost $L$.

\begin{lemma}
    If the original graph $G=(V,E)$ has an independent set of size $k$, then $G'=(V',E')$ has a forbidden subgraph-free $d$-factor of weight $(d+2)|E|L + 3k$.
\end{lemma}



==> 4.linear_hardness.tex <==
\section{ \texorpdfstring{$k$}{}-Node-Augmentation Hardness for \texorpdfstring{$k=o(n)$}{}}

We begin with a weighted Tree Augmentation Instance with tree $T=(V,E)$ with links $L\subseteq \binom{V}{2}$, with costs $c : L \rightarrow \mathbb{R}_{\geq 0}$. In this section we will provide a polynomial time reduction from $(T,L,c)$ to an weighted $k$-node-augmentation instance $G=(V',E')$ with links $F \subseteq \binom{V'}{2}$, and costs $c': L' \rightarrow \mathbb{R}_{\geq 0}$, for any $k \in O(n^{n-\varepsilon})$, for $0<\varepsilon \leq \frac{1}{2}$. 

The reduction is as follows. First, for every node $v\in V$, we will add to $G$ a complete subgraph on $k+1$ nodes, that we denote by $K_v$. For every edge $e\in E$, we will add to $G$ a complete subgraph on $k$ nodes, that we denote by $K_e$. For $e=uv\in E$, we will add to $E'$ the edges of a complete bipartite graph between $K_e$ and $K_v$, and between $K_e$ and $K_u$.

For every link $\ell=uv \in L$, we add a corresponding link $\ell'$ to $L'$ with one endpoint chosen arbitrarily from $K_u$ and one endpoint chosen arbitrarily from $K_v$. We will then set $c'(\ell') = c(\ell)$.

\begin{lemma}
    The minimum cuts of $G$ are exactly the set $\{K_e | e\in E\}$. That is, each minimum cut corresponds to an edge in $T$.
\end{lemma}
\begin{proof}
    First, we claim that $K_e$ is a cut of $G$ for every $e\in E$. Assume that $G \backslash K_e$ is connected for some $e=uv \in E$. Then there is a path from $K_u$ to $K_v$ in $G$. The edges in $G$ are either in the complete subgraphs corresponding to edges and nodes in $T$ or, for node $v\in V$ there are edges from $K_v$ to $K_ef$ for any edge $f\in E$ that has $v$ as an endpoint. Therefore, if $G\backslash K_e$ is connected, then there is a path between $K_u$ and $K_v$ that alternates between node subgraphs and edge subgraphs. Thus, by construction of $G$ that must mean there is a path from $u$ to $v$ in $T-\{e\}$, which contradicts that $T$ is a tree.

    So for every $e\in E$, $K_e$ is a cut and therefore the size of a minimum cut in $G$ is at most $k$. Consider any two nodes $x,y\in V'$, it is not hard to see that there are at least $k$ internally disjoint paths between $x$ and $y$ in $G$. Thus the size of a minimum cut is at least $k$, and thus is equal to $k$.
    
    Assume for the sake of contradiction that there is a minimum cut $C$ that is not equal to $K_e$ for some $e\in E$.
    Consider two nodes $x,y\in V'$ separated by $C$. Clearly, $x$ and $y$ are not part of the same $K_v$ or $K_e$ for $v\in V$ or $e\in E$ as they would be adjacent. Similarly, if (wlog) $x$ is in $K_v$ for some $v$, then $y$ cannot by in $K_e$ for some $e=uv \in E$.

    Suppose $x\in K_u$ and $ y\in K_v$ for $u,v\in V$, and let $u=u_0,e_1,u_1, \dots, e_m,u_m = v$ be the path in $T$ between $u$ and $v$. By construction of $G$, every minimum path from $x$ to $y$ must be within $\bigcup_{i=0}^m K_{u_i} \cup \bigcup_{i=1}^m K_{e_i}$. Since $C$ is a minimum cut that separates $x$ and $y$, $C \subsetneq \bigcup_{i=0}^m K_{u_i} \cup \bigcup_{i=1}^m K_{e_i}$. 
    
    Suppose $C \cap K_{u_i} \neq \emptyset$ for some $i=1,\dots,m-1$, it is clear that since $|C| < |K_{u_i}|$, there is a path from $K_{e_i}$ to $K_{e_{i+1}}$ in $G \backslash C$. Thus, $C$ is not a minimum cut as $C \backslash K_{u_i}$ would still separate $x$ and $y$. Therefore, $C\subsetneq \bigcup_{i=1}^m K_{e_i}$. However, by a similar argument $C$ cannot be a minimum cut since $C$ cannot equal any $K_{e_i}$ by assumption on $C$. Therefore, $C$ cannot be a minimum cut, contradicting our assumption on $C$.
\end{proof}

\begin{lemma}
    Given a feasible solution $F' \subseteq F$ to the $k$-node-augmentation instance $(G,F',c)$, $L' \coloneqq \{ \ell =uv \in L | \exists \ell' \in F \text{ with endpoints in } K_u \text{ and } K_v\}$ is a feasible solution to the weighted TAP instance $(T,L,c)$ with cost $c(L') = c'(F')$.
\end{lemma}
\begin{proof}
    First, it is clear that $c(L') = c'(F')$ by definition of $F$. 

    Assume for the sake of contradiction that $L'$ is not a feasible solution to the Weighted TAP instance $(T,L,c)$. That is, there is a bridge $e=uv\in E$ of $T\cup L'$, so there are no links in $L'$ with endpoints in both of the components of $T\backslash\{e\}$. Therefore, there must be no links in $F'$ with endpoints in both of the components of $G\backslash \{K_e\}$, and $K_e$ is a cut of size $k$, which is a contradiction to the feasibility of $F'$. 
\end{proof}

\begin{lemma}
    Given a feasible solution $L'\subseteq L$ to the Weighted TAP instance $(T,L,c)$, $F' = \{ \ell ' \in F | uv \in L \text{ and } \ell ' \text{ has endpoints in } K_u \text{ and } K_v \}$ is a feasible solution to the $k$-node-augmentation instance $(G,F,c')$, and $c'(F') = c(L')$.
\end{lemma}
\begin{proof}
    First, it is clear that $c(L') = c'(F')$ by definition of $F$.

    Assume for the sake of contradiction that $F'$ is not a feasible solution to the $(G,F,c')$ instance. That is, there is a minimum cut of $G\cup F'$ of size $k$. We know such cuts are the subgraphs $K_e$ for some $e\in E$. In particular, there is no link in $F'$ with endpoints on both sides of $G\backslash K_e$. Therefore, there are no link in $L'$ with endpoints on both sides of $T\backslash\{e\}$, so $L'$ is infeasible, which is a contradiction. 
\end{proof}


